Allo: A Programming Model for Composable Accelerator Design

Special-purpose hardware accelerators are increasingly pivotal for sustaining performance improvements in emerging applications, especially as the benefits of technology scaling continue to diminish. However, designers currently lack effective tools and methodologies to construct complex, high-performance accelerator architectures in a productive manner. Existing high-level synthesis (HLS) tools often require intrusive source-level changes to attain satisfactory quality of results. Despite the introduction of several new accelerator design languages (ADLs) aiming to enhance or replace HLS, their advantages are more evident in relatively simple applications with a single kernel. Existing ADLs prove less effective for realistic hierarchical designs with multiple kernels, even if the design hierarchy is flattened. In this paper, we introduce Allo, a composable programming model for efficient spatial accelerator design. Allo decouples hardware customizations, including compute, memory, communication, and data type from algorithm specification, and encapsulates them as a set of customization primitives. Allo preserves the hierarchical structure of an input program by combining customizations from different functions in a bottom-up, type-safe manner. This approach facilitates holistic optimizations that span across function boundaries. We conduct comprehensive experiments on commonly-used HLS benchmarks and several realistic deep learning models. Our evaluation shows that Allo can outperform state-of-the-art HLS tools and ADLs on all test cases in the PolyBench. For the GPT2 model, the inference latency of the Allo generated accelerator is 1.7x faster than the NVIDIA A100 GPU with 5.4x higher energy efficiency, demonstrating the capability of Allo to handle large-scale designs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.03.  Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> code/bit_operation.tex <==
\begin{center}
\vspace{3pt}
\begin{minipage}{0.55\linewidth}
\begin{minted}[linenos,
               fontsize=\small]{python}
# bit slicing
a: int40 = 0xabcd0123
>>> a[28:32] # containing the bit of 28-31
0xa
\end{minted}
\end{minipage}
\begin{minipage}{0.2\linewidth}
\begin{minted}[linenos,
               fontsize=\small]{python}
# bit indexing (popcount)
sum: int32 = 0
for i in range(a.width):
    sum += a[i]
\end{minted}
\end{minipage}
\vspace{3pt}
\end{center}

==> code/external_ip.tex <==
\begin{figure}[!htbp]
\begin{minipage}{0.52\linewidth}
\begin{minted}[linenos,
               xleftmargin=\parindent,
               fontsize=\scriptsize]{python}
gemm = allo.load_ip(
  top="gemm", headers=["gemm.h"], impls=["gemm.cpp"]
)
def kernel(A: int32[32][32], B: int32[32][32])
           -> int32[32][32]:
  C: int32[32][32] = 0
  gemm(A, B, C, 32, 32, 32)
  return C
\end{minted}
\end{minipage}
\begin{minipage}{0.43\linewidth}
\begin{minted}[linenos,
               fontsize=\scriptsize]{cpp}
// gemm.cpp, given by HLS libraries
template<typename T>
void gemm(hls::stream<T>& A, hls::stream<T>& B,
          hls::stream<T>& C,
          const uint64_t p_m, const uint64_t p_n,
          const uint64_t p_k) {
    // high-performance implementation...
}
\end{minted}
\end{minipage}
\caption{An example of importing external IP modules to a \Name kernel.}
\label{fig:external_ip}
\end{figure}

==> code/systolic_def.tex <==
\begin{figure}[!htbp]
\begin{minipage}{0.5\linewidth}
\begin{minted}[linenos,
               xleftmargin=\parindent,
               fontsize=\scriptsize]{python}
def PE(
    A_in: int8[K], B_in: int8[K],
    A_out: int8[K], B_out: int8[K],
    C: int16[M, N], i: index, j: index,
):
    v: int16 = 0
    for k in range(K):
        a: int8 = A_in[k]
        b: int8 = B_in[k]
        v += a * b
        A_out[k] = a
        B_out[k] = b
    C[i, j] = v
\end{minted}
\end{minipage}
\begin{minipage}{0.45\linewidth}
\begin{minted}[linenos,
               fontsize=\scriptsize]{python}
def systolic(A: int8[M, K], B: int8[K, N],
             C: int16[M, N]):
    A_reg: int8[M, N + 1, K]
    B_reg: int8[N, M + 1, K]
    A_reg[:M, 0, :K] = A[:M, :K]
    B_reg[:N, 0, :K] = B[:K, :N]
    for i, j in allo.grid(M, N, name="PE"):
        PE(
            A_reg[i, j], B_reg[j, i],
            A_reg[i, j + 1], B_reg[j, i + 1],
            C, i, j
        )
    # ... data drain
\end{minted}
\end{minipage}
\caption{A specification of an output-stationary systolic array~\cite{kung1978systolic} for the GEMM kernel.}
\label{fig:systolic_def}
\end{figure}

==> code/systolic_equ.tex <==
\begin{figure}[!htbp]
\begin{minipage}{0.5\linewidth}
% \small
\begin{align*}
&\text{Input}  &&\text{operations} &\\
&a(i,j,k)      &&= A_{ik}\,, & 1\leq i\leq M, j=0, 1\leq k\leq K\\
&b(i,j,k)      &&= B_{kj}\,, & i=0, 1\leq j\leq N, 1\leq k\leq K\\
&c(i,j,k)      &&= 0     \,, & 1\leq i\leq M, 1\leq j\leq N, k=0\\
&\text{Output} &&\text{operations} &\\
&C_{ij}        &&= c(i,j,k)\,,& 1\leq i\leq M, 1\leq j\leq N, k=K\,
\end{align*}
\end{minipage}
% \hfill
\hfill\vline\hfill
\begin{minipage}{0.4\linewidth}
% \small
\begin{align*}
\text{Calculations}\\
a(i,j,k) &= a(i,j-1,k)\\
b(i,j,k) &= b(i-1,j,k)\\
c(i,j,k) &= c(i,j,k-1)\\
         &+ a(i,j-1,k)\cdot b(i-1,j,k)\\
1\leq i\leq M, &1\leq j\leq N, 1\leq k\leq K
\end{align*}
\end{minipage}
\caption{Recurrence equation of an output-stationary systolic array~\cite{kung1978systolic}.}
\label{fig:systolic_equ}
\end{figure}
% https://gyires.inf.unideb.hu/KMITT/a52/ch04.html

==> code/systolic_mlir.tex <==
\begin{figure}[!htbp]
% \begin{minipage}{0.95\linewidth}
\begin{minted}[xleftmargin=\parindent,
               fontsize=\scriptsize]{java}
module {
  func.func @PE(%arg0: memref<8xi8, strided<[1], offset: ?>>, %arg1: memref<8xi8, strided<[1], offset: ?>>,
                %arg2: memref<8xi8, strided<[1], offset: ?>>, %arg3: memref<8xi8, strided<[1], offset: ?>>,
                %arg4: memref<8x8xi16>, %arg5: index, %arg6: index)
  func.func @systolic(%arg0: memref<8x8xi8>, %arg1: memref<8x8xi8>, %arg2: memref<8x8xi16>) {
    %alloc = memref.alloc() {name = "A_reg"} : memref<8x9x8xi8>
    %alloc_0 = memref.alloc() {name = "B_reg"} : memref<8x9x8xi8>
    // initialization
    affine.for %arg3 = 0 to 8 {
      affine.for %arg4 = 0 to 8 {
        // ...
        func.call @PE(%subview, %subview_3, %subview_4, %subview_6, %arg2, %arg3, %arg4)
      } {loop_name = "j"}
    } {loop_name = "i", op_name = "PE"}
    // ... store back results
    return
}}
\end{minted}
% \end{minipage}
\caption{\MLIR representation of the systolic function in Fig.~\ref{fig:systolic_def}.}
\label{fig:mlir_systolic}
\end{figure}

==> code/typing_fixed.tex <==
% \begin{figure}[!htbp]
% \begin{mathpar}
% \texttt{arith} ::= \,\texttt{add}\, | \,\texttt{sub}\, | \,\texttt{mul}\, | \,\texttt{div}\,| \,\texttt{min}\, |\,\texttt{max}\, \\
% \texttt{cmp} ::= \,\texttt{eq}\, | \,\texttt{ne}\, | \,\texttt{slt}\, | \,\texttt{sle}\, |\,\texttt{sgt}\, |\,\texttt{sge}\, |\,\texttt{ult}\, |\,\texttt{ule}\, | \,\texttt{ugt}\, |\,\texttt{uge}\\
% % subtype
% \infer[SubType]{\textbf{ufixed}_{w, f} < \textbf{fixed}_{w, f}}{} \qquad
% % fixed add, sub, mul, div
% \infer[FixedArith]{\Gamma \vdash \texttt{arith}\, e_{1},e_{2} : \textbf{fixed}_{w, f}}{\Gamma \vdash e_{1} : \textbf{fixed}_{w,f} \quad \Gamma \vdash e_{2} : \textbf{fixed}_{w,f}} \\
% % fixed cmp
% \infer[FixedCmp]{\Gamma \vdash e_{1} \,\texttt{cmp}\, e_{2} : \textbf{i1}}{\Gamma \vdash e_{1} : \textbf{fixed}_{w,f} \quad \Gamma \vdash e_{2} : \textbf{fixed}_{w,f}} \qquad
% % cast
% \infer[FixedCast]{\Gamma \vdash \texttt{cast}\,e : \textbf{fixed}_{w_2,\,f_2}}{\Gamma \vdash e : \textbf{fixed}_{w_2,\,f_2} \quad \Gamma \vdash \texttt{cast} : \textbf{fixed}_{w_1,\,f_1} \rightarrow \textbf{fixed}_{w_2,\,f_2}}
% \end{mathpar}
% \caption{Typing rules of fixed-point arithmetic operations.}
% \label{fig:typing_fixed}
% \end{figure}

\begin{figure}[!htbp]
\begin{mathpar}
\infer[FixedAdd]{\Gamma \vdash e_{1} : \textbf{fixed}_{w_1,f_1} \quad \Gamma \vdash e_{2} : \textbf{fixed}_{w_2,f_2}}{\Gamma \vdash \texttt{add}\, e_{1},e_{2} : \textbf{fixed}_{\max(w_1-f_1,w_2-f_2)+\max(f_1,f_2)+1,\,\max(f_1,f_2)}} \quad
\infer[FixedMul]{\Gamma \vdash e_{1} : \textbf{fixed}_{w_1,f_1} \quad \Gamma \vdash e_{2} : \textbf{fixed}_{w_2,f_2}}{\Gamma \vdash \texttt{mul}\, e_{1},e_{2} : \textbf{fixed}_{w_1+w_2,\,f_1+f_2}}\\
\infer[FixedSelect]{\Gamma \vdash e_{1} : \textbf{int1} \quad \Gamma \vdash e_{2} : \textbf{fixed}_{w_1,f_1} \quad \Gamma \vdash e_{3} : \textbf{fixed}_{w_2,f_2}}{\Gamma \vdash e_{2}\; \texttt{if}\; e_{1}\; \texttt{else}\; e_{3} : \textbf{fixed}_{\max(w_1-f_1,w_2-f_2)+\max(f_1,f_2),\,\max(f_1,f_2)}}
\end{mathpar}
\caption{Typing rules of example fixed-point operations. $\textbf{fixed}_{w,f}$ represents a fixed-point type with $w$ bits in total and $f$ fractional bits.}
\label{fig:typing_fixed}
\end{figure}


==> code/typing_shape.tex <==
\begin{figure}[!htbp]
\begin{mathpar}
\infer[Broadcasting]{\Gamma \vdash e_{1} : shape(a_{N_1},\ldots,a_0) \quad \Gamma \vdash e_{2} : shape(b_{N_2},\ldots,b_0)\quad \forall i\in\{1,\ldots,N_2\},a_i=b_i\lor a_i=1\lor b_i=1}{\Gamma \vdash \texttt{op}(e_1,e_2) : shape(a_{N_1},\ldots,\max(a_{N_2}, b_{N_2}),\ldots,\max(a_0,b_0))}
\end{mathpar}
\caption{Shape inference rule. Suppose $N_1>N_2$. \texttt{op} is element-wise operations.}
\label{fig:typing_shape}
\end{figure}

==> code/typing_struct.tex <==
\begin{figure}[!htbp]
\begin{mathpar}
\infer[Construct]{\Gamma \vdash \texttt{struct}(e_1, e_2, ..., e_n) : \tau_1 \times \tau_2 \times ... \times \tau_n}{\Gamma \vdash e_1 : \tau_1 \quad \Gamma \vdash e_2 : \tau_2 \quad ... \quad  \Gamma \vdash e_n : \tau_n} \qquad
\infer[Access]{\Gamma \vdash \texttt{struct\_acc}(e,\,i) : \tau_i}{\Gamma \vdash e : \tau_1 \times \tau_2 \times ... \times \tau_n \quad \Gamma \vdash i : \textbf{i32}}
\end{mathpar}
\caption{Typing rules of struct operations.}
\label{typing:struct}
\end{figure}

==> sections/x-compilation.tex <==
\subsection{Type System}
\label{sub:types}


\subsubsection{Customized Data Types.}
When it comes to arbitrary bitwidth integers, users can declare them using \code{int} or \code{uint}.
\Name provides support for bit indexing and bit slicing of integers, enabling the implementation of highly efficient bit manipulation algorithms such as \texttt{popcount} in hardware, as demonstrated in the following code snippet:

\input{code/bit_operation}

For fixed-point numbers, users can specify a fixed-point type with \code{fixed(width, frac)}, where \code{width} represents the overall data bitwidth, and \code{frac} denotes the number of fractional bits.
During CPU simulation (\S\ref{sub:codegen}), these quantized data types are automatically converted to integers.

Furthermore, \Name extends its support to user-defined struct types. Users can define a struct type by providing a dictionary that specifies the base type for each field. For instance, the code below declares a point struct type with two fields of \code{int8}:
\begin{center}
\code{stype = allo.Struct({"x": int8, "y": int8})}
\end{center}

This feature allows users to define custom data structures tailored to their specific hardware design requirements, enhancing the flexibility and expressiveness of \Name.

\subsubsection{Type Inference.}

Furthermore, partial access to the arrays is also supported for enhanced flexibility.
For instance, in Line 9 of the \code{systolic} function, only the first two dimensions of the 3D array \code{A_reg} are accessed, resulting in a 1D array for the \code{PE} function input.
Currently, \Name supports static shape inference, while dynamic shapes and symbolic shape inference are planned as part of our future work.

\subsection{IR Builder}
\label{sub:ir_builder}
We construct our intermediate representation in \MLIR~\cite{chris2021mlir}, a modular compiler infrastructure that enables different optimizations performed at different levels of abstraction.
The \MLIR ecosystem offers a rich collection of built-in dialects, with each dialect comprising a set of \MLIR operations that serve as the fundamental building blocks for constructing complex programs.
Each \MLIR operation is denoted in the following format:
\begin{center}
    \mintinline{python}{<dialect>.<operation>(<operands>) <attributes> : <type> {<regions>}}
\end{center}
An operation may have multiple operands and an optional attribute map, and it can have several regions, each of which contains multiple blocks.
Operations can be recursively nested within blocks.

Fig.\ref{fig:mlir_systolic} presents an example of the \MLIR representation derived from Fig.\ref{fig:systolic_def}.
In this figure, the \texttt{func} dialect is utilized to depict function definitions and function calls.
The \texttt{memref} dialect is employed for representing multi-dimensional arrays.
Beyond the basic element types and shapes, \texttt{memref} types can also include additional layout and memory space information, which will be annotated later when performing memory customizations such as array partitioning and streaming.
The \texttt{affine} dialect is responsible for describing the nested \texttt{for} loop within the program, with attached \texttt{loop\_name} and \texttt{op\_name} attributes for subsequent references.

\input{code/systolic_mlir}

We can see from Fig.~\ref{fig:mlir_systolic} that we strictly follow the program structure captured by the AST, preserving the hierarchical program structure when constructing the IR.
This hierarchical structure is subsequently passed down to the hardware code generation phase, ensuring that the module information is retained.
While the actual computation details are not depicted in this figure, we incorporate automatic data type casting logic in the program based on the typing rules outlined in \S\ref{sub:types}.
Users are relieved of the need to manage the intricacies of type casting for intermediate variables.

\subsection{Scheduler}
\label{sub:scheduler}

We decouple the hardware customizations from the algorithm specification and introduce an \Name dialect within \MLIR to represent each of the primitives.
The various primitives that \Name supports are detailed in Table~\ref{tab:primitives}.
Apart from the compute customizations specific to nested loops, \Name further provide memory and communication customizations for designing high-performance hardware accelerator.
By decoupling these customizations at the IR level, \Name gains the flexibility to support a wider range of programs.
As long as a program can be expressed within the \MLIR framework, it can use the \Name dialect for program transformation.

Unlike TVM~\cite{chen2018tvm} and HeteroCL~\cite{lai2019heterocl} that represent primitives as a set of compiler passes, \Name inherits the idea from Exo~\cite{yuka2022exo} and TensorIR~\cite{feng2022tir} that treat each primitive as a rewrite to the program.
This approach allows for immediate, incremental transformation of the program.
Primitives are applied successively, enabling users to directly observe the impact of each transformation without the need to wait for all the primitives to be collectively executed.
We further extend this decoupling idea to support memory banking and multi-kernel composition, which are not supported by previous works~\cite{yuka2022exo,chen2018tvm}.
Details will be discussed \S\ref{sec:composition}.


==> sections/x-example.tex <==
\section{Motivating Example}
\label{sec:movtivation}

\subsection{Scheduling a GEMM Kernel}
\label{sub:alg_spec}

\input{code/allo_gemm}
Although the row-wise product GEMM can have good performance for small kernels, if we want to further scale up the design, we need to leverage a more efficient implementation for the GEMM kernel, and systolic array~\cite{kung1978systolic} is one of them.

% While certain hardware DSLs like Pylog~\cite{huang2021pylog} also leverage native Python grammar for accelerator generation, they do not mandate users to provide explicit data type annotations but instead attempt to infer them from the input data.
% However, this approach presents certain limitations.
% First, it limits users' control over the data types of intermediate variables, which can be crucial in scenarios where, for example, a variable like \code{v} in the left side of Fig.~\ref{fig:systolic_def} must be a high bitwidth integer to prevent overflow.
% Second, it may not support parameterized or composite data types, which are essential for constructing highly modular kernel libraries.

\subsection{Schedule Construction}

\subsubsection{Memory Customization.}
After reordering the reduction loop (\code{k}) with the non-reduction loop (\code{j}), we can employ the \code{.buffer_at()} primitive to create a line buffer called \code{buf_C} for the output \code{C} (Line 6).
This can be viewed as creating an additional memory hierarchy, where the results are initially written to \code{buf_C}.
Upon the completion of the target loop iteration, the results are then transferred from \code{buf_C} to off-chip memory.
The buffer size is automatically determined by the compiler to ensure the correctness of the results.

Furthermore, we offer a \code{.partition()} primitive for partitioning the array into multiple banks (Lines 7-9), so that the elements can be accessed in parallel.
Notice array partitioning is essentially changing the data layout and will have a significant impact on the function interface.
Further discussions regarding layout composition can be found in Section~\ref{sub:partition}.

From this example, we can see \Name can replicate the optimized row-wise product in Fig.~\ref{fig:single_hls} in less than 10 lines of schedule code.
This approach does not need to alter the original GEMM implementation, greatly enhancing the productivity in designing hardware accelerators.


We begin by considering the matrix multiplication operation: $C_{ij}=\sum_k A_{ik}B_{kj}$, where $1\leq i\leq M, 1\leq j\leq N, 1\leq k\leq K$.
Our goal is to construct an output-stationary systolic array of size $M\times N$ to compute $C_{ij}$.
In this configuration, input tensors $A$ and $B$ are fed through distinct PEs, and the output value accumulates within each PE across the time dimension.
To explicitly represent the computations occurring within each PE and model data reuse across the time dimension, we create a sequence of instances $c(i,j,k)$ that represents the state of $c(i,j)$ at timestamp $k$.
A similar approach is applied to $a(i,j,k)$ and $b(i,j,k)$.
This formulation provides a behavioral specification for a systolic array, as depicted in Fig.~\ref{fig:systolic_equ}.
Here, $a$, $b$, and $c$ function as registers within each PE, facilitating data storage and transmission.

% \input{code/systolic_equ}

To realize this system of equations, we further segregate the spatial and temporal dimensions.
Spatial dimensions, like $i$ and $j$, are responsible for mapping computations to different PEs executing concurrently, while temporal dimensions, such as $k$, describe the computations taking place within each PE at each time step.
Notice certain efforts~\cite{wang2021autosa} have aimed to automate the space-time transformation.
However, this specific aspect is not the primary focus of our DSL, as our emphasis lies in capturing the hierarchical structure of the computation.

\input{code/systolic_def}

We utilize an output-stationary systolic array as a concrete example to illustrate communication customization in \Name, showcasing its capabilities in handling complex transformations, as demonstrated in Fig.~\ref{fig:systolic_def}.
The compute logic of each processing element (PE) is explicitly defined within the \code{PE} function and subsequently invoked within the top-level \code{systolic} function.
This hierarchical approach cleanly separates the temporal and spatial components of the computation.
In this structured program, each variable must be declared either in the function argument or within a statement accompanied by a type annotation (Lines 1-4 in \code{systolic}).
The syntax is as follows: \code{<name>: <type>[<shape>]}.
Our type system accommodates arbitrary bitwidth integer types, floating points, fixed points, and more details regarding this type system are elaborated in \S\ref{sub:types}.
Notice if only variable declarations are provided (Lines 3-4), the variable will not be automatically initialized with concrete values.
However, users have the flexibility to include an assignment statement if they wish to initialize the array with a specific initial value.

Lines 5-6 initialize the registers as depicted in Fig.\ref{fig:systolic_equ}.
\Name supports slicing and broadcasting operations similar to those in NumPy\cite{harris2020numpy}.
Line 7 iterates through the spatial loop, with \code{allo.grid} serving as syntactic sugar for Python's \code{range} to iterate over a grid of indices.
Within each \code{PE}, a dot-product operation is conducted, and the result is written back to the array \code{C}.

This example illustrates how \Name adeptly manages nested function calls, which are mapped as nested modules in the hardware design.
This hierarchical structure would be challenging to implement without the support of imperative programming.
For instance, neither tensor expressions in TVM~\cite{chen2018tvm} nor HeteroCL~\cite{lai2019heterocl} can adequately represent this intricate structure, since they represent programs in a declarative way that cannot capture the nested function calls.


\subsection{External Libraries}
\label{sub:external_kernels}
In certain cases, simply relying on the \Name kernel library or direct customization within \Name's interface may not suffice.
Many existing HLS-based kernel libraries~\cite{vitis_hls_library,vitis_ai} are available, and to efficiently incorporate these external kernels into \Name, we provide an IP integrator for seamless integration.
As shown in Fig.~\ref{fig:external_ip}, users can make use of the \code{load_ip} function to load an IP from an external library.
By providing the top-level function and necessary implementation files, users can effortlessly integrate the external IP into their \Name design.
After loading, the IP becomes directly callable within the \Name kernel.
Users are only required to specify the correct number of arguments, and \Name will automatically determine the appropriate interface for the IP.
Furthermore, if the interface requires changing the memory layout or implementing a FIFO, Algorithm~\ref{alg:layout} is also used to ensure that the interface remains consistent across different functions.
In cases where the algorithm has been predefined, the \code{.bind(<func>,<ip>)} primitive allows users to bind an IP implementation to an existing kernel function.
This IP integration process is implemented with PyBind11~\cite{pybind11}, with wrapper functions generated automatically by \Name.
As a result, users need not be concerned with low-level implementations.
This makes \Name more general and extensible to different customizations.

\input{code/external_ip}

